On the Rate-Distortion-Complexity Trade-offs of Neural Video Coding

This paper aims to delve into the rate-distortion-complexity trade-offs of modern neural video coding. Recent years have witnessed much research effort being focused on exploring the full potential of neural video coding. Conditional autoencoders have emerged as the mainstream approach to efficient neural video coding. The central theme of conditional autoencoders is to leverage both spatial and temporal information for better conditional coding. However, a recent study indicates that conditional coding may suffer from information bottlenecks, potentially performing worse than traditional residual coding. To address this issue, recent conditional coding methods incorporate a large number of high-resolution features as the condition signal, leading to a considerable increase in the number of multiply-accumulate operations, memory footprint, and model size. Taking DCVC as the common code base, we investigate how the newly proposed conditional residual coding, an emerging new school of thought, and its variants may strike a better balance among rate, distortion, and complexity.

==> Section/2_related.tex <==
\section{Related Work}
\label{sec:related}


==> Table/BD.tex <==
\begin{table*}[]
\caption{BD-rate (\%) comparison measured in PSNR-RGB. The anchor is conditional coding with $C=64$.}
\vspace{-0.1cm}
\label{table:BD}
\centering
\begin{tabular}{l|cccccc|c}
\toprule
                         & UVG & HEVC-B & HEVC-C & HEVC-E & HEVC-RGB & MCL-JCV &  Average \\
\midrule                         
Cond. (C=64)             &      0 &      0 &      0 &      0 &      0 &      0 &       0  \\
Cond. Res. (C=64)        &   -1.3 &   -2.5 &   -3.3 &   -2.4 &   -2.0 &   -1.4 &    -2.15 \\
Masked Cond. Res. (C=64) &   -8.6 &   -7.3 &   -7.9 &  -13.6 &   -6.2 &   -4.6 &    -8.03 \\
\midrule
Cond. (C=32)             &    6.5 &    9.7 &   18.8 &   13.2 &    7.8 &    8.6 &    10.77 \\
Cond. Res. (C=32)        &   -0.8 &   -0.5 &    4.9 &   -3.5 &   -0.6 &    0.0 &    -0.08 \\
Masked Cond. Res. (C=32) &   -5.1 &   -4.7 &    0.2 &  -10.3 &   -3.0 &   -2.1 &    -4.17 \\
\midrule
Cond. (C=16)             &    7.3 &   12.3 &   22.6 &    9.0 &   10.7 &   14.0 &    12.65 \\
Cond. Res. (C=16)        &    0.3 &    1.0 &    7.4 &   -3.1 &    2.6 &    3.3 &     1.92 \\
Masked Cond. Res. (C=16) &   -3.9 &   -4.1 &    1.4 &  -10.8 &   -3.0 &   -1.2 &    -3.60 \\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table}[]
% \caption{BD-rate comparison. The anchor is conditional coding with 64 channels conditioning signal.}
% \centering
% \begin{tabular}{lcccc}
% \hline
%                          & UVG & HEVC-B & MCL-JCV & Avg. \\
% \hline                         
% Cond. (C=64)             &     &         &        &      \\
% Cond. Res. (C=64)        &     &         &        &      \\
% Masked Cond. Res. (C=64) &     &         &        &      \\
% \hline
% Cond. (C=32)             &     &         &        &      \\
% Cond. Res. (C=32)        &     &         &        &      \\
% Masked Cond. Res. (C=32) &     &         &        &      \\
% \hline
% Cond. (C=16)             &     &         &        &      \\
% Cond. Res. (C=16)        &     &         &        &      \\
% Masked Cond. Res. (C=16) &     &         &        &      \\
% \hline
% \end{tabular}
% \end{table}

%                          & UVG & HEVC-RGB & MCL-JCV & HEVC-B & HEVC-C & HEVC-E & Average \\
% \midrule                         
% Cond. (C=64)             &      0 &      0 &      0 &      0 &      0 &      0 &     0  \\
% Cond. Res. (C=64)        &   -1.3 &   -2.0 &   -1.4 &   -2.5 &   -3.3 &   -2.4 &  -2.15 \\
% Masked Cond. Res. (C=64) &   -8.6 &   -6.2 &   -4.6 &   -7.3 &   -7.9 &  -13.6 &  -8.03 \\
% \midrule
% Cond. (C=32)             &    6.5 &    7.8 &    8.6 &    9.7 &   18.8 &   13.2 &  10.77 \\
% Cond. Res. (C=32)        &   -0.8 &   -0.6 &    0.0 &   -0.5 &    4.9 &   -3.5 &  -0.08 \\
% Masked Cond. Res. (C=32) &   -5.1 &   -3.0 &   -2.1 &   -4.7 &    0.2 &  -10.3 &  -4.17 \\
% \midrule
% Cond. (C=16)             &    7.3 &   10.7 &   14.0 &   12.3 &   22.6 &    9.0 &  12.65 \\
% Cond. Res. (C=16)        &    0.3 &    2.6 &    3.3 &    1.0 &    7.4 &   -3.1 &   1.92 \\
% Masked Cond. Res. (C=16) &   -3.9 &   -3.0 &   -1.2 &   -4.1 &    1.4 &  -10.8 &  -3.60 \\

==> Table/BD_BT709.tex <==
\begin{table*}[]
\caption{BD-rate (\%) comparison with the distortion measured in the PSNR-RGB domain. The anchor is conditional coding with $C=64$.}
\vspace{-0.1cm}
\label{table:BD_BT709}
\centering
\begin{tabular}{l|cccccc|c}
\toprule
                         & UVG & HEVC-B & HEVC-C & HEVC-E & HEVC-RGB & MCL-JCV &  Average \\
\midrule                         
Cond. (C=64)             &      0 &      0 &      0 &      0 &      0 &      0 &       0  \\
Cond. Res. (C=64)        &   -1.8 &   -2.4 &   -2.9 &   -1.8 &   -2.0 &   -2.0 &    -2.15 \\
Masked Cond. Res. (C=64) &  -10.3 &   -7.7 &   -7.5 &  -14.3 &   -6.2 &   -6.0 &    -8.67 \\
\midrule
Cond. (C=32)             &    5.5 &    8.3 &   17.9 &   11.4 &    7.8 &    7.5 &     9.73 \\
Cond. Res. (C=32)        &   -2.0 &   -1.3 &    4.4 &   -5.3 &   -0.6 &   -0.7 &    -0.92 \\
Masked Cond. Res. (C=32) &   -5.8 &   -5.3 &    0.5 &  -11.7 &   -3.0 &   -3.1 &    -4.73 \\
\midrule
Cond. (C=16)             &    6.1 &   10.6 &   21.0 &    7.2 &   10.7 &   12.4 &    11.33 \\
Cond. Res. (C=16)        &    0.0 &    0.2 &    6.3 &   -3.5 &    2.6 &    2.5 &     1.35 \\
Masked Cond. Res. (C=16) &   -5.1 &   -4.9 &    0.1 &  -11.9 &   -3.0 &   -2.6 &    -4.57 \\
\bottomrule
\end{tabular}
\end{table*}

==> Table/BD_BT709_piece_wise.tex <==
\begin{table*}[]
\caption{BD-rate (\%) comparison with the distortion measured in the PSNR-RGB domain. The anchor is conditional coding with $C=64$.}
\vspace{-0.1cm}
\label{table:BD_BT709_piece_wise}
\centering
\begin{tabular}{l|cccccc|c}
\toprule
                         & UVG & HEVC-B & HEVC-C & HEVC-E & HEVC-RGB & MCL-JCV &  Average \\
\midrule                         
Cond. (C=64)             &     0  &     0  &     0  &      0  &     0  &     0  &       0  \\
Cond. Res. (C=64)        &  -1.93 &  -2.43 &  -3.16 &   -1.81 &  -2.13 &  -2.03 &    -2.25 \\
Masked Cond. Res. (C=64) & -10.28 &  -7.73 &  -7.72 &  -14.36 &  -6.18 &  -5.91 &    -8.70 \\
\midrule
Cond. (C=32)             &   5.36 &   8.12 &  17.05 &   11.30 &   7.54 &   7.50 &     9.48 \\
Cond. Res. (C=32)        &  -2.00 &  -1.19 &   4.34 &   -5.13 &  -0.73 &  -0.51 &    -0.87 \\
Masked Cond. Res. (C=32) &  -5.90 &  -5.31 &   0.26 &  -11.87 &  -3.31 &  -3.07 &    -4.87 \\
\midrule
Cond. (C=16)             &   6.04 &  10.53 &  20.61 &    7.07 &  10.55 &  12.47 &    11.21 \\
Cond. Res. (C=16)        &  -0.16 &   0.09 &   5.62 &   -3.81 &   2.29 &   2.49 &     1.09 \\
Masked Cond. Res. (C=16) &  -5.11 &  -4.96 &  -0.11 &  -11.76 &  -3.16 &  -2.48 &    -4.60 \\
\bottomrule
\end{tabular}
\end{table*}

==> Table/BD_traditional.tex <==
\begin{table*}[]
\caption{Traditional BD-rate (\%) comparison. The anchor is conditional coding with 64 channels conditioning signal.}
\label{table:RD traditional}
\centering
\begin{tabular}{l|cccccc|c}
\toprule  
                         & UVG & HEVC-RGB & MCL-JCV & HEVC-B & HEVC-C & HEVC-E & Average \\
\midrule                         
Cond. (C=64)             &      0 &      0 &      0 &      0 &      0 &      0 &     0  \\
Cond. Res. (C=64)        &   -0.8 &   -2.6 &   -5.1 &   -2.6 &   -3.3 &   -2.6 &  -2.83 \\
Masked Cond. Res. (C=64) &   -9.6 &   -8.5 &   -0.0 &   -7.3 &   -7.7 &  -13.8 &  -7.82 \\
\midrule
Cond. (C=32)             &    8.4 &    4.7 &    5.9 &    9.1 &   18.2 &   12.9 &   9.87 \\
Cond. Res. (C=32)        &    0.3 &   -3.2 &   -4.7 &   -0.9 &    4.4 &   -3.8 &  -1.32 \\
Masked Cond. Res. (C=32) &   -4.7 &   -6.2 &   -5.0 &   -4.6 &   -0.1 &  -10.5 &  -5.18 \\
\midrule
Cond. (C=16)             &    8.1 &    6.0 &    9.8 &   11.4 &   21.9 &    8.7 &  10.98 \\
Cond. Res. (C=16)        &    1.5 &   -1.4 &    4.1 &    0.3 &    7.3 &   -3.4 &   1.40 \\
Masked Cond. Res. (C=16) &   -4.1 &   -6.6 &   -2.7 &   -4.5 &    1.2 &  -11.2 &  -4.65 \\
\bottomrule
\end{tabular}
\end{table*}

==> Table/training.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Training procedure. MENet, FE, 3x3 Conv represent the motion estimation network, the feature extractor, and the 3x3 Conv in Fig.~\ref{fig:schemes}, respectively. EPA is the error propagation aware training in \cite{EPA}.}
\begin{tabular}{cccccccccc}
\hline
\multirow{2}{*}{Phase}               & \multicolumn{5}{c}{Training Modules}                                 & \multirow{2}{*}{Number of Frames} & \multirow{2}{*}{Epoch} & \multirow{2}{*}{lr} \\ \cline{2-6}
                                     & MENet & Motion Codec & FE \& 3x3 Conv & Inter-frame Codec & Mask Generator &                               &             &           \\ \hline
Motion Coding                        &       & v            &          &                   &                & 3                             & -           & 1e-4            \\ \hline
Motion Compensation                  &       &              & v        &                   &                & 3                             & 2          & 1e-4            \\ \hline
\multirow{2}{*}{Inter-frame Coding}  &       &              & v        & v                 & v              & 3                             & 4          & 1e-4            \\ \ 
                                     &       &              & v        & v                 & v              & 5                             & 4          & 1e-4            \\ \hline
\multirow{2}{*}{Finetuning}          &       & v            & v        & v                 & v              & 3                             & 3          & 1e-4            \\ \ 
                                     &       & v            & v        & v                 & v              & 5                             & 3          & 1e-4            \\ \hline
\multirow{2}{*}{Finetuning with EPA} &       & v            & v        & v                 & v              & 5                             & 2          & 1e-5            \\ \ 
                                     & v     & v            & v        & v                 & v              & 5                             & 2          & 1e-5            \\ \hline
\end{tabular}
\end{table*}

==> Table/training_origin.tex <==
\begin{table*}[t!]
\centering
\caption{\textcolor{blue}{Training procedure. MENet, MWNet, MCNet represent the motion estimation network, the motion extrapolation network, and the motion compensation network, respectively. EPA is the error propagation aware training in \cite{EPA}.}}
\label{tab:training}
\begin{tabular}{ccllcc}

\hline
\textcolor{blue}{Phase}                                                      & \textcolor{blue}{Number of Frames} & \textcolor{blue}{Training Modules}                      & \textcolor{blue}{Loss}                                                             & \textcolor{blue}{lr}   & \textcolor{blue}{Epoch} \\
\hline
\textcolor{blue}{Motion Coding}                                              & \textcolor{blue}{3}                & \textcolor{blue}{MWNet and motion codec}                & \textcolor{blue}{$R^{motion}_t + \lambda \times D(x_t, warp(x_{t-1}, \hat{f}_t))$}   & \textcolor{blue}{1e-4} & \textcolor{blue}{10}     \\\hline
\textcolor{blue}{Motion Compensation}                                        & \textcolor{blue}{3}                & \textcolor{blue}{MCNet}                                 & \textcolor{blue}{$R^{motion}_t + \lambda \times D(x_t, \hat{x}_c)$}                  & \textcolor{blue}{1e-4} & \textcolor{blue}{5}      \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textcolor{blue}{Inter-frame Coding}}}    & \textcolor{blue}{3}                & \textcolor{blue}{Inter-frame codec and mask generator}  & \textcolor{blue}{$R_t + \lambda \times D(x_t, \hat{x}_t)$}                           & \textcolor{blue}{1e-4} & \textcolor{blue}{10}     \\
\multicolumn{1}{c}{}                                                         & \textcolor{blue}{5}                & \textcolor{blue}{Inter-frame codec and mask generator}  & \textcolor{blue}{$R_t + \lambda \times D(x_t, \hat{x}_t)$}                           & \textcolor{blue}{1e-4} & \textcolor{blue}{5}     \\\hline
\textcolor{blue}{Finetuning}                                                 & \textcolor{blue}{5}                & \textcolor{blue}{All modules except MENet}             & \textcolor{blue}{$R_t + \lambda \times D(x_t, \hat{x}_t)$}                           & \textcolor{blue}{1e-4} & \textcolor{blue}{3}     \\\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textcolor{blue}{Finetuning with EPA}}}   & \textcolor{blue}{5}                & \textcolor{blue}{All modules except MENet}             & \textcolor{blue}{$R_t + \lambda \times D(x_t, \hat{x}_t)$}                           & \textcolor{blue}{1e-4} & \textcolor{blue}{3}     \\
\multicolumn{1}{c}{}                                                         & \textcolor{blue}{5}                & \textcolor{blue}{All modules}                          & \textcolor{blue}{$R_t + \lambda \times D(x_t, \hat{x}_t)$}                           & \textcolor{blue}{1e-5} & \textcolor{blue}{3}     \\\hline
\end{tabular}
\end{table*}

% \begin{table}[]
% \begin{tabular}{lllllll}
% Phase                                                  & \# of Frames & Frozen Module                                         & Training Modules          & Loss            & lr   & Epochs \\
% Load pre-trained                                       &             & load pretrained MENet and  MWNet                      &                           &                 &      &        \\
% Motion coding                                          & 3           & MENet                                                 & MWNet and motion codec    & $R_{motion} + \lambda \times(x_t, warp(x_{t-1}, \hat{f}_t)$ & 1e-4 & 10     \\
% MCNet                                                  & 3           & MENet, MWNet, motion codec                            & MCNet                     & $\lambda D + R$ & 1e-4 & 5      \\
% Inter coding                                           & 3           & \multicolumn{1}{c}{MENet, MWNet, motion codec, MCNet} & Inter-frame codec         & $\lambda D + R$ & 1e-4 & 10     \\
% \multicolumn{1}{c}{}                                   & 5           & \multicolumn{1}{c}{MENet, MWNet, motion codec, MCNet} & Inter-frame codec         & $\lambda D + R$ & 1e-4 & 5      \\
% Finetune                                               & 5           & MENet                                                 & All networks except MENet & $\lambda D + R$ & 1e-4 & 3      \\
% \multicolumn{1}{c}{\multirow{2}{*}{Finetune with EPA}} & 5           & MENet                                                 & All networks except MENet & $\lambda D + R$ & 1e-4 & 3      \\
% \multicolumn{1}{c}{}                                   & 5           &                                                       & All networks              & $\lambda D + R$ & 1e-5 & 3     
% \end{tabular}
% \end{table}

==> Table/training_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\label{table:training2}
\centering
\caption{Training procedure. MENet, FE, 3x3 Conv represent the motion estimation network, the feature extractor, and the 3x3 Conv in Fig.~\ref{fig:schemes}, respectively. Inter-frame Codec in this table represents the refinement net, $\{G^{enc}, G^{dec}\}$, and the frame generator in Fig.~\ref{fig:schemes}. EPA is the error propagation aware training in \cite{EPA}.}
\setlength\tabcolsep{3.95pt}
\begin{tabular}{ccccccccccc}
\hline
\multirow{2}{*}{Phase}               & \multirow{2}{*}{Step} & \multicolumn{5}{c}{Training Modules}                                                                                                                                                                                                                 & \multirow{2}{*}{Training Objective}                              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# of \\ Frames\end{tabular}} & \multirow{2}{*}{Epoch} & \multirow{2}{*}{lr} \\ \cline{3-7}
                                     &                       & \begin{tabular}[c]{@{}c@{}}Inter-frame\\ Codec\end{tabular} & MENet & \begin{tabular}[c]{@{}c@{}}Motion \\ Codec\end{tabular} & \begin{tabular}[c]{@{}c@{}}FE \& \\ 3x3 Conv\end{tabular} & \begin{tabular}[c]{@{}c@{}}Mask\\ Generator\end{tabular} &                                                                  &                                                                          &                        &                     \\ \hline
% Motion Coding                        & 1                     &                                                             &       & v                                                       &                                                           &                                                          & $R^{motion}_t+ \lambda \times D(x_t, warp(x_{t-1}, \hat{f}_t)) $ & 3                                                                        & -                      & 1e-4                \\ \hline
Motion Compensation                  & 1                     &                                                             &       &                                                         & v                                                         &                                                          & $R^{motion}_t + \lambda \times D(x_t, \dot{x}_c)$                & 3                                                                        & 2                      & 1e-4                \\ \hline
\multirow{2}{*}{Inter-frame Coding}  & 2                     & v                                                           &       &                                                         & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 3                                                                        & 4                      & 1e-4                \\ \cline{2-11} 
                                     & 3                     & v                                                           &       &                                                         & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 5                                                                        & 4                      & 1e-4                \\ \hline
\multirow{2}{*}{Finetuning}          & 4                     & v                                                           &       & v                                                       & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 3                                                                        & 3                      & 1e-4                \\ \cline{2-11} 
                                     & 5                     & v                                                           &       & v                                                       & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 5                                                                        & 3                      & 1e-4                \\ \hline
\multirow{2}{*}{Finetuning with EPA} & 6                     & v                                                           &       & v                                                       & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 5                                                                        & 2                      & 1e-5                \\ \cline{2-11} 
                                     & 7                     & v                                                           & v     & v                                                       & v                                                         & v                                                        & $R_t + \lambda \times D(x_t, \hat{x}_t)$                         & 5                                                                        & 2                      & 1e-5                \\ \hline
\end{tabular}
\end{table*}
